Interpretable Summaries of Black Box Incident Triaging with Subgroup Discovery

The need of predictive maintenance comes with an increasing number of incidents reported by monitoring systems and equipment/software users. In the front line, on-call engineers (OCEs) have to quickly assess the degree of severity of an incident and decide which service to contact for corrective actions. To automate these decisions, several predictive models have been proposed, but the most efficient models are opaque (say, black box), strongly limiting their adoption. In this paper, we propose an efficient black box model based on 170K incidents reported to our company over the last 7 years and emphasize on the need of automating triage when incidents are massively reported on thousands of servers running our product, an ERP. Recent developments in eXplainable Artificial Intelligence (XAI) help in providing global explanations to the model, but also, and most importantly, with local explanations for each model prediction/outcome. Sadly, providing a human with an explanation for each outcome is not conceivable when dealing with an important number of daily predictions. To address this problem, we propose an original data-mining method rooted in Subgroup Discovery, a pattern mining technique with the natural ability to group objects that share similar explanations of their black box predictions and provide a description for each group. We evaluate this approach and present our preliminary results which give us good hope towards an effective OCE's adoption. We believe that this approach provides a new way to address the problem of model agnostic outcome explanation.

==> tex/relatedwork.tex <==
\section{Related work}\label{sec:relatedwork}
We first present existing incident triage methods, and confirm that the best of them use black box models that do not explain their outcomes. We then describe the state of the art of Explainable AI as well as the Subgroup Discovery task, and we show how our approach provides a novel way to address the problem of explaining black box decisions by efficiently exploiting the Subgroup Discovery framework.

\smallbreak
\noindent \textbf{Incident triage.} Several existing methods address the bug-triage problem which focuses on the automatic assignment of bug reports to software developers~\cite{DBLP:conf/icsm/SarkarRB19,DBLP:conf/sigsoft/JeongKZ09,DBLP:conf/sigsoft/LeeHLKJ17}. While this task is similar to incident triage, the incident-triage problem has many characteristics that makes it more complex~\cite{DBLP:conf/icse/0003HLXZHGXDZ19}. For example, incidents happen more often than bugs, and they can be caused by more various factors , e.g., misconfigurations, hardware failures, service unavailable. The seminal paper~\cite{DBLP:conf/icse/0003HLXZHGXDZ19} show that bug-triage techniques are able to correctly assign incident reports to a certain extent, but still need to be further improved. \cite{DBLP:conf/kbse/0003HL0HGXDZ19} proposed a Deep Learning approach that is specific to incident triage, and demonstrated that it significantly outperforms the state-of-the-art bug-triage approach~\cite{DBLP:conf/sigsoft/LeeHLKJ17}. Few other techniques have been also proposed to deal with the specific problem of incident triage~\cite{DBLP:conf/kdd/PhamJDOJ20,DBLP:conf/sigcomm/GaoYMFLBAWLMYA20,wang2021fast}. DeepTriage~\cite{DBLP:conf/kdd/PhamJDOJ20} combines both  conventional machine learning models and DNN in an ensemble method. The common point between all these methods is that they are based on black box models which do not bring any explanation of their output to the user. An important challenge to successfully automate incident triage is to gain practitioners trust who need to understand the reason behind assigning an incident to them. Hence, we believe that it is crucial that an incident triage method explains its recommendations. We are the first to propose an efficient incident-triage method that takes advantage of the high performance of black box models while cohesively explaining groups of its outcomes.


\smallbreak
\noindent \textbf{Explainable AI.} 
The growing popularity of black box prediction models combined with the crucial need of transparency in many decision processes has conducted to an unprecedented interest on explaining these black box models. Some of the proposed methods are \textit{global}, i.e., they aim at explaining the whole internal logic of the black box, while others provide \textit{local} explanations for specific outcomes. Global explanations are generally provided by learning a potentially interpretable model (e.g., decision tree, classification rules) that mimics the predictions of the original black box model~\cite{DBLP:conf/nips/CravenS95,DBLP:conf/aistats/HaraH18,DBLP:journals/kbs/AndrewsDT95,DBLP:conf/kdd/FungSR05,DBLP:journals/pr/KrishnanSB99,DBLP:journals/npl/AugastaK12,johansson2004accuracy,DBLP:journals/titb/HanLYPC15,DBLP:journals/ijon/BarakatB10}. However, it is often not feasible to explain all the logic as the model can be extremely complex.  Thus, most of recent work focus on local methods that explain each outcome of a black box model independently. These methods provide a local explanation for the prediction of a specific object that can only be interpreted locally. Some of these approaches are designed for a specific model such as DNN~\cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/icml/ShrikumarGK17,DBLP:conf/icml/SundararajanTY17,DBLP:conf/eccv/ZeilerF14} and GNN~\cite{DBLP:conf/nips/YingBYZL19}. On the other hand, many other methods~\cite{DBLP:conf/kdd/Ribeiro0G16,DBLP:conf/pakdd/GuidottiMC19,DBLP:journals/corr/abs-1805-10820,DBLP:journals/corr/abs-2002-03746} are able to explain the outcome of any model (model agnostic). They are often based on the generation of a local neighborhood around the object to explain, and on the training of an interpretable model on this neighborhood. The drawback of outcome explanation methods is the large number of provided explanations if applied to a large number of outcomes. Analyzing individual explanations becomes very time consuming for the end-user. Few methods have been proposed to address this issue, by grouping similar explanations into clusters~\cite{DBLP:conf/aies/IbrahimLMP19} or by selecting a subset of representative explanations~\cite{DBLP:conf/kdd/Ribeiro0G16}. These two methods can thus give a picture of the different possible explanations of a model, however, do not provide to the user the contexts in which each explanation holds. Our approach aims to provide not only the subgroup explanations, but also the subgroup descriptions which explicitly contextualize subgroup objects.

\smallbreak
\noindent \textbf{Subgroup Discovery.} 
Subgroup Discovery (SD)~\cite{DBLP:books/mit/fayyadPSU96/Klosgen96,DBLP:journals/widm/Atzmueller15} is a data mining task that aims at identifying interpretable local subgroups that foster some property of interest. A popular case consists in binary subgroup discovery~\cite{DBLP:conf/pkdd/AtzmullerP06,DBLP:journals/jair/GambergerL02,DBLP:journals/jmlr/LavracKFT04}, i.e., finding subgroups where the proportion of a specific target class is significantly higher than expected. Other approaches consider more complex target attributes such as categorical~\cite{DBLP:conf/pkdd/GrosskreutzRW08}, numerical~\cite{DBLP:journals/datamine/LemmerichAP16,DBLP:conf/pakdd/MillotCB20,DBLP:journals/datamine/BoleyGGV17}, and multi-target~\cite{DBLP:conf/icde/LijffijtKDPOB18,DBLP:journals/datamine/DuivesteijnFK16}. Furthermore, many methods have been proposed to generalize Subgroup Discovery to complex data structures, e.g.,  graphs~\cite{DBLP:journals/datamine/DengKLB21,DBLP:journals/ml/LeeuwenBSM16,DBLP:journals/isci/AtzmuellerDM16,DBLP:journals/ml/KaytouePZBR17} and sequential data~\cite{DBLP:conf/iccv/NowozinBT07,DBLP:conf/dsaa/MathonatNBK19,DBLP:journals/eswa/HeZW19,DBLP:journals/isci/HeZGW19}.
%, spatiotemporal data~\cite{centeio2021want,neves2020efficient}, trees and forests~\cite{DBLP:journals/datamine/AdriaensLB19}. 
An important component of Subgroup Discovery is the interestingness measure~\cite{DBLP:journals/csur/GengH06}, which is a function used to assess the quality of the subgroup. This function strongly depends on the target application. 
%Most of the proposed measures aim to identify subgroups that discriminate a target concept, for example, the WRAcc~\cite{DBLP:journals/jmlr/LavracKFT04} and the mutual information. 
Once the subgroup discovery task and the interestingness measure are specified, we need to explore the search space of subgroups to identify the ones that optimize the interestingness measure. 
%This step is challenging as the size of the search space can be extremely large. Consequently, researchers devoted significant effort to design efficient mining algorithms. 
Various mining algorithms have been proposed, some of them return exact results while others are heuristic but generally scale better. 
%Although exact algorithms generally exploit the properties of data structures and the interestingness measure to optimize the search strategy, their scalability remains limited. Other algorithms are heuristic, they enable better scalability but they do not provide the guarantee of completeness. 
Many of these approaches have proven their efficiency in different applications and domains such as physics~\cite{goldsmith2017uncovering}, education~\cite{DBLP:journals/ijdsa/HelalLLEDM19} and neuro-science \cite{DBLP:journals/ploscb/LiconBSMFBGRPKB19}. However, none of existing approaches has exploited this framework for the problem of explaining black box predictions. To make such method efficient, we needed to address several complex challenges related to the mined data structure, the subgroup interestingness, as well as a scalable mining algorithm  which optimizes this interestingness measure that is new in SD.
%including: (1) introduce the data to the SD algorithm in the right format, (2) design the right interestingness measure to identify subgroups that delineate the best cohesive outcome explanations, (3) use/design a mining algorithm that scales while optimizing the chosen interestingness.

